GEANN: Scalable Graph Augmentations for Multi-Horizon Time Series Forecasting

Encoder-decoder deep neural networks have been increasingly studied for multi-horizon time series forecasting, especially in real-world applications. However, to forecast accurately, these sophisticated models typically rely on a large number of time series examples with substantial history. A rapidly growing topic of interest is forecasting time series which lack sufficient historical data -- often referred to as the ``cold start'' problem. In this paper, we introduce a novel yet simple method to address this problem by leveraging graph neural networks (GNNs) as a data augmentation for enhancing the encoder used by such forecasters. These GNN-based features can capture complex inter-series relationships, and their generation process can be optimized end-to-end with the forecasting task. We show that our architecture can use either data-driven or domain knowledge-defined graphs, scaling to incorporate information from multiple very large graphs with millions of nodes. In our target application of demand forecasting for a large e-commerce retailer, we demonstrate on both a small dataset of 100K products and a large dataset with over 2 million products that our method improves overall performance over competitive baseline models. More importantly, we show that it brings substantially more gains to ``cold start'' products such as those newly launched or recently out-of-stock.

==> discussion.tex <==
\subsection{Data-Driven Graph Stability}
\label{app:graph_analysis}
In this paper, we have considered both data-driven and the domain-knowledge defined graph, and we observe that the performance of using a data-driven graph is volatile while the domain-knowledge graph seems to produce consistent improvements across different datasets. In this section, we conduct an in-depth analysis for the data-drive graph used to provide insights for this result.

\paragraph*{\bf Distribution of similarity metrics} We first compare the nearest neighbor distribution for these two graphs, respectively, for the large scale dataset used in Section 3.2. Appendix Figure \ref{fig:knn-stats} depicts a histogram of the estimated means and standard deviations of the Pearson correlations from 10 nearest neighbors for each product in GEANN-kNN. The substantial concentration of mean correlations near unity, and similarly the concentration of standard deviation near zero, show that many of the products have nearly interchangeable rank. On the other hand, Appendix Figure \ref{fig:bw-stats}, which shows a similar histogram of those for co-browsing counts from 10 nearest neighbors for each product in GEANN-bw, presents much stronger variation. Moreover, it is clear that a subset of products have strong similarity relative to others, with mean co-browsing counts above 35.

\paragraph*{\bf On $k$-NN graph volatility} One reason such context-based $k$-NN graphs may show unreliable relationships relevant to forecasts is the stability of the $k$-NN construction on embeddings $\mathbf{H}$. We define stability for a product $a$ and number of neighbors $k$ across runs $r$, each run generating a context $\mathbf{H}^{(r)}$, as
\begin{equation}
    \nonumber
    \begin{aligned}
    \text{Stability}(a ; k, \mathcal{R}) &\equiv \dfrac{\left|\bigcap_{r\in\mathcal{R}} \text{KNN}_{r}(a ; k)\right|}{k}.
    \end{aligned}
\end{equation}
Stability is a measure of preservation of graph similarity across model training runs; a random selection of neighbors has a stability proportional to a HyperGeometric$(N, k, k)$, where $N$ is the number of data observations. When $N$ is reasonably large, the stability is close to 0, and a deterministic graph has a stability of 1.0. Prior work in natural language processing field shows the stability of frequently used word embeddings are often 0.8 or greater \citep{borah2021word}.

Figure \ref{appendix:stability} shows the distribution of stability by the number of neighbors for our embedding based $k$-NN using Pearson correlation across 3 model runs. We find generally low stability of $k$-NN relationships generated from the embeddings $\mathcal{H}$. While the stability of low numbers of neighbors is relatively larger at 0.5, it quickly decreases to represent an approximately random graph as the number of neighbors increases--- likely due to orderings based on correlation being overcome by model noise. Moreover, the stability is highly consistent across products. A maximal stability of approximately 0.5 suggests that the $k$-NN based graph may provide an inconsistent signal due to noise in the embeddings $\mathbf{H}$.
\begin{figure}[H]
    \centering
    \hspace{-.2in}\includegraphics[scale=.55]{figs/pearson_correlation_60neighbors.png}
    \caption{Boxplots of stability by number of neighbors for $k$-NN generated from Pearson correlation between embeddings $\mathbf{H}$ across 3 runs of MQCNN. Blue points represent outliers.}
    \label{appendix:stability}
\end{figure}
